Optimal Transport Posterior Alignment for Cross-lingual Semantic Parsing

Cross-lingual semantic parsing transfers parsing capability from a high-resource language (e.g., English) to low-resource languages with scarce training data. Previous work has primarily considered silver-standard data augmentation or zero-shot methods, however, exploiting few-shot gold data is comparatively unexplored. We propose a new approach to cross-lingual semantic parsing by explicitly minimizing cross-lingual divergence between probabilistic latent variables using Optimal Transport. We demonstrate how this direct guidance improves parsing from natural languages using fewer examples and less training. We evaluate our method on two datasets, MTOP and MultiATIS++SQL, establishing state-of-the-art results under a few-shot cross-lingual regime. Ablation studies further reveal that our method improves performance even without parallel input translations. In addition, we show that our model better captures cross-lingual structure in the latent space to improve semantic representation similarity.

==> tables/ablation_mtop_d_recon.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% {\sc Minotaur}+AE & EN   & FR   & ES   & DE   & HI   & Avg. \\ \midrule
% 1 SPIS          & 80.1$~\pm~$1.6 & 70.7$~\pm~$0.4 & 70.3$~\pm~$1.1 & 67.0$~\pm~$0.5   & 62.5$~\pm~$0.8 & 67.6$~\pm~$3.8 \\
% 5 SPIS          & 76.5$~\pm~$0.2 & 71.4$~\pm~$5.6 & 73.0$~\pm~$3.8   & 68.6$~\pm~$4.9 & 68.2$~\pm~$3.4 & 70.3$~\pm~$2.3 \\
% 10 SPIS & 78.0$~\pm~$0.2 & 72.5$~\pm~$0.5 & 73.5$~\pm~$0.4 & 69.3$~\pm~$0.5 & 68.2$~\pm~$0.6 & 70.9$~\pm~$2.5 \\
% \bottomrule
% \end{tabular}%
% }
% \caption{SCIEM Accuracy on MTOP with {\sc Minotaur}+AE augmenting the model with
% an additional autoencoding objective across SPIS sample rates. {\sc Minotaur}+AE
% performs worse than {\sc Minotaur} with significant penalty ($p<0.01$) at 1\& 5
% SPIS and non-significant penalty at 10 SPIS ($p=0.15$). Overall, the additional
% objective is not required for the latent variable to be semantically informative.}
% \label{tab:ablation:reconloss}
% \end{table}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
 & EN   & FR   & ES   & DE   & HI   & Avg. \\ \midrule
1 SPIS          & 80.1 & 70.7 & 70.3 & 67.0   & 62.5 & 67.6 \\
5 SPIS          & 76.5 & 71.4 & 73.0   & 68.6 & 68.2 & 70.3 \\
10 SPIS & 78.0 & 72.5 & 73.5 & 69.3 & 68.2 & 70.9 \\
\bottomrule
\end{tabular}%
}
\caption{Accuracy on MTOP with {\sc Minotaur}+AE augmenting the model with
an additional autoencoding objective across SPIS sample rates. {\sc Minotaur}+AE
performs worse than {\sc Minotaur} with significant penalty ($p<0.01$) at 1\& 5
SPIS and non-significant penalty at 10 SPIS ($p=0.15$). Overall, the additional
objective is not required for the latent variable to be semantically informative.}
\label{tab:ablation:reconloss}
\end{table}

